Rigorous Evaluation of Microarchitectural Side-Channels with Statistical Model Checking

Rigorous quantitative evaluation of microarchitectural side channels is challenging for two reasons. First, the processors, attacks, and defenses often exhibit probabilistic behaviors. These probabilistic behaviors arise due to natural noise in systems (e.g., from co-running processes), probabilistic side channel attacks, and probabilistic obfuscation defenses. Second, microprocessors are extremely complex. Previous evaluation methods have relied on abstract or simplified models, which are necessarily less detailed than real systems or cycle-by-cycle simulators, and these models may miss important phenomena. Whereas a simple model may suffice for estimating performance, security issues frequently manifest in the details. We address this challenge by introducing Statistical Model Checking (SMC) to the quantitative evaluation of microarchitectural side channels. SMC is a rigorous statistical technique that can process the results of probabilistic experiments and provide statistical guarantees, and it has been used in computing applications that depend heavily on statistical guarantees (e.g., medical implants, vehicular computing). With SMC, we can treat processors as opaque boxes, and we do not have to abstract or simplify them. We demonstrate the effectiveness of SMC through three case studies, in which we experimentally show that SMC can evaluate existing security vulnerabilities and defenses and provide qualitatively similar conclusions with greater statistical rigor, while making no simplifying assumptions or abstractions. We also show that SMC can enable a defender to quantify the amount of noise necessary to have a desired level of confidence that she has reduced an attacker's probability of success to less than a desired threshold, thus providing the defender with an actionable plan for obfuscation via noise injection.

==> OLD-discussion.tex <==
\section{Discussion}
\subsection{Apply SMC to Other Side Channels}
\textcolor{blue}{While we view SMC as a plug-in tool, we claim it can be used for the evaluation of many kinds of side channels with probabilities. Except for the case of unexplored obfuscation defense we have shown, we want to discuss another kind of side channel - The side channel of Network-on-Chip(NoC), to open up the scope of using SMC flexibly.}

\textcolor{blue}{The on-chip mesh interconnect is facing vulnerabilities \cite{dai:security:2022}. The attacker can work by observing secret-dependent interconnect traffic from the victim. However, it's hard to quantify or formally analyze the side channel in NoC. While previous work didn't even build a precise probabilistic model for even one microarchitectural in one core, NoC consists of several cores with routers, on-chip buffers, and other components, which is impossible to build a probabilistic model without simplification. \cite{Li:isca:2024} tries to build a formal model for even a simplified NoC model with Murphi[CITE] to find deadlocks, but it results in using bounded model checking due to the large state space. }


% \subsection{Number of samples to achieve a certain Confidence}
% \textcolor{blue}{While we all want to save efforts in one evaluation to do more iterations, SMC holds one significant advantage -- it doesn't need a huge number of samples to achieve high confidence. To customize SMC in microarchitectural security evaluation, we further discuss the number of samples to achieve 90\%, 95\%, and 99\% confidence in our case studies. As the security researchers would like to see a strong statistical guarantee, SMC provides a path to achieve a 99\% guarantee with a comparatively smaller number of samples. And one can also save effort with only less than 20 samples to achieve a 90\% confidence in relaxed scenarios.  }


% remain for discussion
% \textcolor{blue}{
% Current approaches to security are formulate/discover attack, solve with bespoke defense scheme, and break defense scheme with new attacker avoid defense scheme altogether. \\
% (1) This strategy is too specific to the particular attack/defense scheme under consideration and similar to 'whack-a-mole'. Researchers need to shoulder the load to develop an entirely new defense scheme for each new attack that comes out, and you burden the architecture with taking on the overhead of each new bespoke defense scheme that is added to it. This is not scalable and time-efficient.\\
% (2) If you design a defense scheme for a specific attack, it doesn't protect against other attacks and may negatively interfere with other defense schemes colocated on the machine. For this, we would prefer a defense scheme that is agnostic to the specific attack but secure against any current attack and future attack. The proposed project can require future evaluation on the specific obfuscation, security, performance tradeoffs with new attacks, but its general principals will stand the test of time.
% }


==> prime-probe.tex <==
\section{Case Study 1: Prime + Probe} \label{sec:case1}

We first illustrate the power and potential of SMC in the context of a simple, well-known side channel attack: prime+probe.  Our goal is not to innovate in security, but rather to demonstrate the application of SMC to security.  The innovation lies in not just the use of SMC but also in the development of SMC experiments that provide insight and actionable information.

\subsection{Prime \& Probe in General}

In general, in a prime+probe (P\&P) attack, the attacker first $primes$ the cache by placing its own data in the cache.  The attacker prompts the victim to run (e.g., by making a request to decode an input codeword).  In the course of doing its work, the victim brings its own data into the cache, thus displacing some of the data the attacker had placed there.  Then the attacker $probes$ the cache by reading the data it had originally put in the cache.  Any accesses that take longer than a cache hit indicate blocks that were evicted to make room for the victim's data.  The attacker can thus glean information about the victim by knowing which cache sets the victim accessed.  

There are many variations of the P\&P attack, but they all follow this basic structure.  For our purposes, many details of the attacks are orthogonal to what we are doing here, such as how the attacker determines which virtual addresses map to the same cache set after they have been translated.

\subsection{The Specific Attack}

The victim program is performing AES decryption.  P\&P is applicable to many possible victim applications, but AES is a well-known example.  AES uses a 16-byte key that is the target of the attacker.

The attacker primes the cache, prompts the victim to encrypt a codeword, and then probes the cache.  By performing this P\&P loop (i.e., prime, encrypt, probe) repeatedly, the attacker can determine which cache sets the victim is accessing when it accesses the AES lookup tables.  This cache access information enables the attacker to uncover the secret key at the half-byte granularity.  

\subsection{The Impact of Natural Noise}

In the absence of noise, an attacker can obtain the secret key in only thousands of P\&P iterations~\cite{tromer:jcrypto:2010}.  However,
the introduction of noise makes the attacker's job more difficult.  In this subsection, we consider only "natural" noise, as described in Section~\ref{sec:methodology}.

The added memory accesses are, to the attacker, indistinguishable from accesses made by the victim.  The "noise" accesses can cause the eviction of the attacker's data from the cache, which is then misinterpreted by the attacker as victim behavior.  More frequent noise accesses correspondingly cause more trouble for the attacker. 

We quantify the impact of noise on the attacker with the metric of $accuracy$, which we define as the number of half-bytes correctly obtained divided by the total number of half-bytes in the key (16).  (Note that random guessing does not achieve 50\% accuracy; randomly guessing a 4-bit quantity results in $1/2^4$ accuracy.)

\vspace{0.2cm}

\noindent
\textbf{Experiment 1.1: At a given noise level, is the attacker's accuracy greater than a given threshold?}
Our first property is the simplest.  To evaluate this first property, we fix the number of P\&P iterations (at 1000) and we consider each of the 5 noise levels. 
In Figure~\ref{fig:case1:accuracy-vs-noise}, we plot the results for 3 different SMC proportions.  (E.g., a proportion of 50\% corresponds to the median.)  First, for every given proportion, we show 99\% confidence intervals for each of the 5 noise levels.  It is not surprising that greater noise leads to lesser accuracy, but the use of SMC enables us to rigorously quantify this relationship. 

 \begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/case1-property1.png}
    \caption{Experiment 1.1: P\&P Accuracy vs. Noise Level.}
    \label{fig:case1:accuracy-vs-noise}
\end{figure}

\vspace{0.2cm}

\noindent
\textbf{Experiment 1.2:  For a number of cache replacements in the range (A-B, A+B), is the attacker's accuracy greater than a given threshold?}  This property is strongly correlated with Experiment 1.1, in that increasing noise leads to increasing numbers of cache replacements. 
 We fix the SMC proportion at 0.5 and the confidence at 95\%.  In Figure~\ref{fig:case1:accuracy-vs-replacements}, we show the results for B=5000 and 
 all five noise levels.  At each noise level we choose a value of A such that all samples fall in the range (A-B, A+B). Each noise level corresponds to a color, and the range (A-B, A+B) for each noise level is denoted with a pair of horizontal dashed lines in the color for that noise level.   
 We plot the confidence interval for accuracy for each value of A, as well as the discrete sample values (discrete dots); the number of samples appears smaller than it is because there is so much overlap between them.
As expected, when there are more replacements---because there are more noise accesses leading to replacements)---it is more difficult for the attacker.   

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/case1-property2.png}
    \caption{Experiment 1.2: P\&P Accuracy vs. Number of Cache Replacements}
    \label{fig:case1:accuracy-vs-replacements}
\end{figure}

Figure~\ref{fig:case1:accuracy-vs-replacements} does not just confirm intuition, but is also actionable, because cache replacements can be observed at runtime with performance counters.  A victim can use this graph to drive an algorithm for monitoring replacements and either (a) simply knowing when it is vulnerable, or (b) injecting noise (discussed next) to drive up replacements when the observed number of replacements is low.  

\subsection{Injecting Noise to Obfuscate Side Channel}

While a victim could always blindly inject noise to deter an attack, the results from SMC can inspire a noise injection heuristic that limits how much noise needs to be injected (and thus limits the performance degradation due to injected noise).
The previous graph shows how a victim could inject noise at different levels, but a victim could instead choose to inject noise intermittently.  In both cases the goal is to inject the minimum amount of noise to achieve a confidence in the attacker's accuracy (or lack thereof), because noise injection hurts performance.  

\vspace{0.2cm}

\noindent
\textbf{Experiment 1.3: If the victim injects noise in a fraction of loops that is in the range (A-B, A+B), is the attacker's accuracy greater than a given threshold?}
In Figure~\ref{fig:case1:accuracy-vs-noise-frequency}, we plot the results for B=15 (a parameter that can be chosen by the victim), with A as the free variable on the x-axis. For example, when A=50, we are considering the situation in which the victim injects noise in 35-65\% of the loops.
We fix the confidence at 90\%.  These results can be used to inform a defense in which noise is not injected all the time.  For example, if A is only 60\%, the confidence interval for median accuracy is still less than 50\%.  

We constructed Figure~\ref{fig:case1:accuracy-vs-noise-frequency} by iterating on a threshold along the x-axis. Because of the high computational cost of simulation in Experiments 1.3 (and later 3.2), we separate the data within a window to use all data within an equidistant upper and lower bound away from the iterated threshold. However, because Experiments 1.4 and 1.5 have a lower computational cost for individual data, we will be able to iterate on a threshold and sample data that exactly matches it. Both sampling techniques separate the data along the x-axis in ways that are useful for analysis.

Using the data we sampled and separated along the x-axis, we iterate along the y-axis to construct accuracy confidence intervals using SMC with the same technique proposed by \cite{mazurek:micro:2023}. We call this method of presenting relationships with a 2-dimensional confidence interval a \textit{tunnel graph}. It is important to note that the graph is discrete in both dimensions at a specified granularity. A smaller granularity improves the continuity of the tunnel graph but increases the required number of simulations.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/case1-property3.png}
    \caption{Experiment 1.3: P\&P Accuracy vs. Frequency of Noise Injection. We create a tunnel graph to evaluate the relationship between obfuscation and accuracy.}
    \label{fig:case1:accuracy-vs-noise-frequency}
\end{figure}

\subsection{The Impact of Probabilistic Cache Behavior}

Cache replacement policies can introduce a measure of probabilistic behavior, and we now explore the impact of this probabilistic behavior on the attacker's success.  Because the probabilistic behavior depends on the cache's set associativity, we consider 2, 4, and 8-way associative caches.

First, though, we set the baseline by considering caches with the deterministic LRU replacement policy. 
 We re-evaluate Experiment 1.1, but for caches with different associativities, and the results are in Figure~\ref{fig:case1:lru_associativity}. We observe that the attack is far more successful on the 8-way and 4-way caches, compared to the 2-way cache.  The intuition for this result is that, for a fixed size cache, less associativity implies more sets. With more sets to consider, it is harder for the attacker to identify an eviction set.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/lru_associativity.png}
    \caption{Attack Accuracy v. noise level for LRU caches of different associativities.}
\label{fig:case1:lru_associativity}
\end{figure}

 \begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/case1-property4.png}
    \caption{Experiment 1.4: P\&P Iterations vs. Accuracy, LRU vs NMRU. We create 2 tunnel graphs for LRU and NMRU accuracy evaluation.}
    \label{fig:c1-p4}
\end{figure}

 \vspace{0.2cm}
\noindent
\textbf{Experiment 1.4: At a fixed noise level, after X iterations, is the accuracy greater than a threshold?}
Now we compare 8-way caches with LRU and NMRU replacement.  With NMRU, among the not-most-recently-used blocks in the set, the cache chooses the victim randomly.  This introduces probabilistic behavior that is more pronounced with greater associativity. (Consider the extreme case of a fully-associative cache, in which NMRU randomly chooses a victim from any block, except the LRU block, in the entire cache.)  We fix the noise level (at the low level of 1) and explore the relationship between the number of P\&P iterations and accuracy. Figure~\ref{fig:c1-p4} shows that NMRU replacement has a significant impact on the attack accuracy.  With LRU, an attacker needs only about 2000 P\&P iterations to be 95\% confident of 100\% accuracy; with NMRU, even 10,000 P\&P iterations does not achieve comparable accuracy.

\vspace{0.2cm}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/nmru-vs-lru-numsamples.png}
    \caption{Experiment 1.5: How many more P\&P iterations are required for NMRU to achieve same accuracy as LRU. We create a tunnel graph to evaluate the relationship between LRU and NMRU iterations.}
    \label{fig:nmru-vs-lru-fixed-accuracy}
\end{figure}
\noindent
\textbf{Experiment 1.5: If after X iterations with an LRU cache the accuracy is A, will it take more than M*X iterations with the NMRU cache to achieve accuracy greater than A?}
Another way of thinking about the difference between LRU and NMRU is to see how many more P\&P iterations are required for an attack on an NMRU cache to be as accurate as an attack on an LRU cache.  We
show these results in Figure~\ref{fig:nmru-vs-lru-fixed-accuracy}. We plot 90\% confidence intervals for $M$, such that performing $MX$ iterations with NMRU achieves the accuracy of $X$ iterations with LRU.  We can make a few observations from these results.  First, the difference between LRU and NMRU decreases until a plateau at around 8,000 iterations.  This results is effectively a different visualization of what we saw in the previous property.  Second, the confidence interval is very large for small numbers of iterations but fairly quickly decreases and converges to a steady-state until about 9,000 iterations, at which point it decrease to another steady-state.  This second observation is not as readily obvious from the evaluation of the prior property.






\subsection{Conclusions from Case Study 1}

In this first case atudy, we have intentionally chosen 
the well-studied security issue of Prime and Probe.  In the context of P\&P, we have shown the power of SMC to provide greater statistical rigor and additional insights.  In doing so, we built no simplifying models and made no assumptions about probability distributions.
Our results here do not upend conventional wisdom, but they confirm---and expand upon---the community's understanding of P\&P. 

%\textcolor{blue}{By Case Study 1, we have shown SMC can expressively give flexible properties to provide insights into the probabilistic behaviors of the attack very rigorously without any simplifications on cache structure. We choose the classic example of the P\&P attack on AES because it's well-understood and people can crystal clearly see how we address this classic problem from SMC's view.}
%\textcolor{red}{Number of samples? Save the effort to build probabilistic model? -- mentioned in case3}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{isca2023-latex-template/figures/case1-property5.png}
%    \caption{Sample number \& accuracy of 8-way NMRU vs. 8-way LRU}
%    \label{fig:c1-p5}
%\end{figure}
